Interactive Summarization and Exploration of Top Aggregate Query Answers

We present a system for summarization and interactive exploration of high-valued aggregate query answers to make a large set of possible answers more informative to the user. Our system outputs a set of clusters on the high-valued query answers showing their common properties such that the clusters are diverse as much as possible to avoid repeating information, and cover a certain number of top original answers as indicated by the user. Further, the system facilitates interactive exploration of the query answers by helping the user (i) choose combinations of parameters for clustering, (ii) inspect the clusters as well as the elements they contain, and (iii) visualize how changes in parameters affect clustering. We define optimization problems, study their complexity, explore properties of the solutions investigating the semi-lattice structure on the clusters, and propose efficient algorithms and optimizations to achieve these goals. We evaluate our techniques experimentally and discuss our prototype with a graphical user interface that facilitates this interactive exploration. A user study is conducted to evaluate the usability of our approach.

==> complexity.tex <==
\section{Complexity Analysis}\label{sec:complexity}
%\red{need to revise this section later - now focus on the heuristic and experiments}
In this section, we discuss the complexity of the problem. If the size limit $k$ is a constant, the problem can be solved in polynomial time. This is because we can iterate over all possible subsets of the clusters of size at most $k$, check if they form a feasible solution, and then return the one with the maximum average value (for \maxval) or with the minimum number of redundant elements (for \minsize). However, this does not give us an efficient algorithm in practice. For example, if $k=10$, the domain size of each attribute is 9, and the number of attributes is 4, the number of clusters (say $N$) can be $10^{4}$, and the number of subsets will be of the order of $N^k = 10^{40}$. Therefore, our goal is to find efficient algorithms that ideally run in polynomial time of $k$ as well. In this section, we treat $k$ as an input parameter. In our experiments, we will compare our algorithms with the brute force method. %% (given in Algorithm \ref{instance of problem}). 
\par
The complexity of the problem may arise due to any of the four factors in Definition~\ref{def:problem}: the size constraint $k$, the coverage parameter $L$, the distance parameter $D$, and the incomparability requirement that the output clusters should form an antichain. Due to multiple constraints, it is not surprising that in general, even checking if there is a non-trivial feasible solution is NP-hard. 
In particular, when $k \leq L$, simply the  requirement of covering $L$ original elements by $k$ clusters in a feasible solution lead to NP-hardness without any other constraints. However, in the case when $k \geq L$ (the user is willing to see $L$ clusters in the top layer of the solution), the decision and the optimization problems become relatively easier. In this section, we show the following for both \maxval\ and \minsize\ objectives. (note that $D = 0$ implies that there is no diversity constraint; the maximum value of $D$ can be $m-1$ according to Definition~\ref{def:distance}); all proofs appear in the full version \cite{fullversion}.
%%
\begin{itemize} %[leftmargin=*]
\itemsep0em
\item $k \geq L$, $D = 0$:~ Top-$k$ elements give the optimal solution, %(Proposition~\ref{prop:top-k-no-D} and 
%(proof in full version \cite{fullversion}), %Appendix~\ref{app:prop:top-k-no-D}), 
since adding any redundant element worsens both the \maxval\ and the \minsize\ objectives.
 %(Case I, Section~\ref{sec:k-geq-L-D-0}).
\item $k \geq L$, arbitrary $D$:~ A non-trivial feasible solution always exists,
%(Proposition~\ref{prop:feasible-exists} and proof in full version \cite{fullversion}): %Appendix~\ref{app:prop:feasible-exists}):
since we can pick arbitrary ancestors of each top-$L$ element from level $D-1$ satisfying all the constraints.  
However, the optimization problems are NP-hard. %(Theorem~\ref{thm:opt-NP-hard}). %(Case II, Section~\ref{sec:k-geq-L-D-arbit}).
\item $k < L$, $D = 0$:~ Even checking  whether a non-trivial feasible solution exists is NP-hard.
% (Theorem~\ref{thm:decision-nphard}). %(Case III, Section~\ref{sec:k-lt-L-D-0}).
\item $k < L$, arbitrary $D$: The same hardness as above holds.
\end{itemize}
%%
Indeed, the optimization problems, even the decision problem of finding a non-trivial solution for $k < L$, might appear at least as hard as the \emph{set cover} problem (given a set of elements and subsets, find the minimum number of subsets that can cover all elements), which is known to be NP-hard, and therefore NP-hardness results are as expected. However, an arbitrary instance of the set cover problem may not give us a valid instance of the lattice structure required in or problem. For a reduction, we need to construct an instance of our ranking problem by creating a set of attributes and assign their values to form a set of tuples in a database. Further, we need to ensure that the `sets' in this reduction conform to a semi-lattice structure. To achieve this, we give reductions from the \textbf{tripartite  vertex cover} problem that is known to be NP-hard \cite{LlewellynTT93}, and construct instances $S$ with only $m  = 3$ attributes. The NP-hardness proof the optimization problem for $k \geq L$ is more involved than the NP-hardness proof for the decision problem for $k < L$, since in the former case the coverage constraint with $k \geq L$ does not lead to the hardness.

%of Theorem~\ref{thm:opt-NP-hard} is more involved than that of Theorem~\ref{thm:decision-nphard}, since in the former the coverage constraint with $k \geq L$ does not lead to the hardness.



\cut{
%%%%%%================= DO NOT DELETE!!!!!! ====================================

\cut{%appendix
\begin{proposition}\label{prop:feasible-exists}
For $k \geq L$ and non-zero $D$, a non-trivial feasible solution always exists.  (proof in Appendix~\ref{app:prop:feasible-exists})
\end{proposition}

\begin{proof}
For each of the top-$L$ elements, pick one of its ancestors at level $D-1$). Let us call this set of clusters $\soln_L$. Clearly, $\soln_L$ covers the top-$L$ elements and has size $\leq L \leq k$ (two top-$L$ elements may pick the same ancestor). Any two clusters in level $D-1$ (and therefore in $\soln_L$) are incomparable  and have distance $\geq D$ (from Proposition~\ref{prop:clusters-at-same-level}). Hence $\soln_{L}$ is a feasible solution.
\end{proof}
}

For $k \geq L$, although finding a feasible solution is easy (Proposition~\ref{prop:feasible-exists}), %However, even for $k \geq L$, 
the optimization problems for both \maxval\ and \minsize\  are NP-hard for an arbitrary value of $D$. Indeed, the optimization problem, even the decision problem of finding a non-trivial solution for $k < L$, might appear at least as hard as the \emph{set cover} problem (given a set of elements and subsets, find the minimum number of subsets that can cover all elements), which is known to be NP-hard. However, for a reduction, we need to create a set of attributes and assign their values to form a set of tuples in a database. Here we give reductions from the \emph{tripartite  vertex cover} problem that is known to be NP-hard\footnote{\cite{GolabKLSS15} gives a reduction from the tri-partite vertex cover problem for \emph{size-constrained weighted set cover} (given weights on the subsets, a size constraint $k$, a coverage fraction $s$, the goal is to return up to $k$ sets that together contain at least $sn$ elements and whose sum of weights is \emph{minimal}). In contrast, in our setting, the weights are assigned on elements (not on subsets); the goal is to select at most $k$ subsets with \emph{maximum} value with the distance and other restrictions,  that cover top-$L$ original  elements; and we show NP-hardness of the decision problem even if the elements are unweighted.}.
\begin{theorem}\label{thm:opt-NP-hard}
The optimization problems for the objectives of \maxval\ and \minsize\ for the case when $k \geq L$ and $D > 0$ is NP-hard. (proof in full version \cite{fullversion}). %Appendix~\ref{app:thm:opt-NP-hard})
\end{theorem}
\cut{%appendix
\begin{proof}
The reduction is from the problem of finding a minimum vertex cover in a tri-partitite graph %(called the \emph{VC-TPG} problem) 
$G$ with partitions $(X, Y, Z)$, which has shown to be NP-hard in \cite{..}. The goal in this problem %in  VC-TPG 
is to decide if the input graph has a vertex cover of size $\leq M$, \ie, a subset of vertices $T \subseteq X \cup Y \cup Z$ and  $|S| \leq M$ such that any edge in $G$ has at least one endpoint in $T$. First we give the proof for {\bf \maxval}. Suppose $G$ has $N_e$ edges and $N_v$ vertices.
\par
Given such a graph $G$ and a bound $M$, we construct a database instance $S$ as follows. There are three attributes $A_X, A_Y, A_Z$.
% and three special values of these attributes $x_0, y_0, z_0$ that do not belong to the set of vertices in $G$. 
(i) \emph{Top-$L$ tuples from the edges of $G$:} Any edge of the form $(x, y), x \in X, y \in Y$ forms two tuples $(x, y, Z^1_{xy})$ and $(x, y, Z^2_{xy})$, where $Z^1_{xy}, Z^2_{xy}$ are two unique values of the $A_Z$ attribute for the edge $(x, y)$ in $G$. Similarly, an edge $(y, z), y\in Y, z \in Z$ forms two tuples $(X^1_{yz}, y, z)$, $(X^2_{yz}, y, z)$, and an edge $(x, z), x \in X, z \in Z$ forms a tuple $(x, Y^1_{xz}, z)$. $(x, Y^2_{xz}, z)$. The weights of these tuples are 1. (ii) \emph{Redundant  tuples from the  vertices of $G$:} For any vertex $x \in A_X$ in $G$, create a redundant tuple $(x, \gamma^2_{x}, \gamma^3_{x})$. These redundant tuples have weight 0. Similarly, form redundant tuples for vertices $y \in A_Y$: $(\gamma^1_{y}, y, \gamma^3_{y})$, and for vertices $z \in A_Z$: $(\gamma^1_{z}, \gamma^2_{z}, z)$ with weight 0. 
(iii) \emph{More redundant  tuples:} For each $Z^1_{xy}$, form $N_r = 2*N_e *N_v$ redundant tuples of the form $(-, -, Z^1_{xy})$ with weight 0, where the positions with $-$ are filled with unique attribute values. Similarly, form redundant $N$ tuples for each of $Z^2_{xy}, Y^1_{xz}, Y^2_{xz}, X^1_{xz}$, and $X^2_{yz}$, placing these attribute values in their corresponding positions.
\par
 We set $k = M$, $L = 2 \times N_e$, $D = 3$. Note that only the tuples from the edges of the form $(x, y, Z^1_{xy}), (x, y, Z^2_{xy}), (x, Y^1_{xz}, z), (x, Y^2_{xz}, z), (X^1_{yz}, y, z), (X^2_{yz}, y, z)$ form the top-$L$ original elements and have to be covered. We claim that $G$ has a vertex cover of size $\leq M$ if and only if $S$ has a solution, a set of clusters $SC$, of value $\geq \frac{2N_e}{2N_e + M}$, where $N_e$ is the number of edges in $G$.
\par
(only if) Suppose $G$ has a vertex cover $T$ of size $M' \leq M$. For any $x \in X \cap T$, choose the cluster $(x, *, *)$ in $SC$; similarly for $y \in Y \cap T$ and $z \in Z \cap T$, choose the clusters $(*, y, *)$ or $(*, *, z)$ respectively in $SC$. These clusters have mutual distance $= 3$, are incomparable, have size $\leq M$, and cover all top-$L$ elements. Each such cluster also covers a redundant element (with $\gamma$ attribute value) of value 0. Therefore, the value of the solution is $\frac{2N_e \times 1 + M' \times 0}{2N_e + M'} \geq \frac{2N_e}{2N_e + M}$. 
\par
(if) Suppose $S$ has a solution $SC$ of value $\geq \frac{2N_e}{2N_e + M}$. Without loss of generality, any cluster in $SC$ covers at least one of the top-$L$ elements with value 1, otherwise it can be discarded without increasing the value of the average or size/distance/coverage of the solution (the redundant elements have value 0 and can only reduce the average). Also note that the trivial solution $(*,*, *)$ cannot be chosen, since it has value $\frac{2N_e + 0}{2N_e + N_v + 2N_e * N_r} $ $\leq \frac{2N_e}{2N_e + 2N_e * N_r}$ $= \frac{1}{1 + N_r} = \frac{1}{1 + 2N_e N_v}$, which is strictly less than the assumed value of $SC$ $\geq \frac{2N_e}{2N_e + M}$. 
\par
\emph{(A) None of the chosen clusters in $SC$ can be of the form  $(*, *, Z^1_{xy})$ (similarly for $Z^2_{xy}, Y^1_{xz}, Y^2_{xz}, X^1_{xz}$).} Suppose one cluster in $SC$ is $(*, *, Z^1_{xy})$. Then it covers $N_r$ redundant tuples that are not covered by any other cluster in $SC$. Suppose $SC$ has $N'$ redundant tuples all together from all other clusters. Then the average value of $SC$ is $\frac{2N_e + 0}{2N_e + N' + N_r}$ $\leq \frac{2N_e}{2N_e + N_r}$ $= \frac{2N_e}{2N_e + 2N_e N_v}$ = $\frac{1}{1 + N_v}$, which is strictly less than $\frac{2N_e}{2N_e + M}$, the assumed value of $SC$ since $M \leq N_v$.
\par
Next we argue that each cluster in $SC$ can have exactly two $*$-s, combining with (A) above, must be of the form $(x, *, *), (*, y, *), (*,*, z)$.
\par
\emph{(B) The clusters in $SC$ cannot have zero $*$-s.} Suppose without loss of generality that for a top-$L$ tuple  $(x, y, Z^1_{xy})$, the singleton cluster  $(x, y, Z^1_{xy})$ has been chosen in $SC$. Due to the incomparability condition, none of $(x, y, *), (x, *, *), (*, y, *)$ can belong to $SC$. Hence, to cover the other top-$L$ tuple $(x, y, Z^2_{xy})$, one of $(x, y, Z^2_{xy}), (x, *, Z^2_{xy}), (*, y, Z^2_{xy})$ has to be chosen $(*, *, Z^2_{xy})$ cannot be chosen due to (A) above. However, these three clusters have distance 1, 2, 2 respectively from $(x, y, Z^1_{xy})$ violating the distance constraint $D = 3$.
\par
\emph{(C) The clusters in $SC$ cannot have one $*$-s.} (i) Suppose for a top-$L$ tuple  $(x, y, Z^1_{xy})$, the cluster  $(x, y, *)$ has been chosen in $SC$. Due to the incomparability condition, none of $(x, *, *), (*, y, *)$ can belong to $SC$, and any cluster with 1 or zero $*$ to cover top-$L$ tuples from edges of the form $(x, y')$ or $(x', y)$ in $G$ will have distance $\leq 2$ with $(x, y, *)$, violating $D = 3$. If $(x, *, Z^1_{xy})$ is chosen (same for $(*, y, Z^1_{xy})$), to cover the other top-$L$ tuple $(x, y, Z^2_{xy})$, one of $(x, y, Z^2_{xy}), (x, *, Z^2_{xy}), (*, y, Z^2_{xy})$ has to be chosen. Since the first two have distance 1 and 2 respectively from $(x, *, Z^1_{xy})$ violating the distance constraint $D = 3$, $(*, y, Z^2_{xy}$ must also belong to $SC$. However, $(x, *, Z^1_{xy})$ and $(*, y, Z^2_{xy})$ together rule out covering clusters for other top-$L$ tuples from edges of the form $(x, y')$ or $(x', y)$ in $G$, which will have distance $\leq 2$ from either of these two clusters, violating $D = 3$.
\par
Hence the clusters in $SC$ must be of the form $(x, *, *)$, $(*, y, *)$, or $(*, *, z)$, which corresponds to a vertex cover in $G$. Suppose there are $K$ clusters in $SC$. Then the value of $SC$ is $\frac{2N_e + 0}{2N_e + K} \geq \frac{2N_e}{2N_e + M}$ by our assumption, hence $K \leq M$, and $G$ has a vertex cover of size at most $M$.
\par
The proof for \textbf{\minsize} is almost the same and simpler, where we argue that $G$ has a vertex cover of size $M$ if and only if $S$ has a feasible solution $SC$ covering $M$ redundant elements. 
\end{proof}
}

%\subsection{Case III: {$k < L$, $D = 0$}}\label{sec:k-lt-L-D-0}
Unlike the case when $k \geq L$, if there are fewer clusters than the desired number of top elements to be covered $k < L$, even the decision version becomes NP-hard.



\begin{theorem}\label{thm:decision-nphard}
The decision version of whether a feasible non-trivial solution exists for the problem defined in Definition~\ref{def:problem} is NP-hard,even with three attributes, $D = 0$, $L = n$, and uniform weights of the elements\footnote{The top-$k$ original elements may not constitute an optimal solution for $D = 0$ when $L > k$.} (proof in full version \cite{fullversion}). % Appendix~\ref{app:thm:decision-nphard})
\end{theorem}
\cut{%appendix
\begin{proof}[of Theorem~\ref{thm:decision-nphard}]
The reduction is again from the problem of finding a minimum vertex cover in a tri-partitite graph %(called the \emph{VC-TPG} problem) 
$G$ with partitions $(X, Y, Z)$ (see the proof of Theorem~{thm:opt-NP-hard}).
\cut{
 which has shown to be NP-hard in \cite{..}. The goal in this problem %in  VC-TPG 
is to decide if the input graph has a vertex cover of size $\leq M$, \ie, a subset of vertices $T \subseteq X \cup Y \cup Z$ and  $|S| \leq M$ such that any edge in $G$ has at least one endpoint in $T$.
}
\par
Given such a graph $G$ and a bound $M$, we construct a database instance $S$ as follows. There are three attributes $A_X, A_Y, A_Z$.
% and three special values of these attributes $x_0, y_0, z_0$ that do not belong to the set of vertices in $G$. 
Any edge of the form $(x, y), x \in X, y \in Y$ forms a tuple $(x, y, Z_{xy})$, where $Z_{xy}$ is a unique value of the $A_Z$ attribute for the edge $(x, y)$ in $G$. Similarly, an edge $(y, z), y\in Y, z \in Z$ forms a tuple $(X_{yz}, y, z)$, and an edge $(x, z), x \in X, z \in Z$ forms a tuple $(x, Y_{xz}, z)$. The total number of tuples in the relation $S$ is $n$ and each tuple has the same weight $1$. We set $k = M$, $L = $ the number of edges in $G$, and claim that $G$ has a vertex cover of size $\leq M$ if and only if $S$ has a non-trivial solution, a set of clusters $SC$, of size $\leq k$.
\par
(only if) Suppose $G$ has a vertex cover $T$ of size $\leq M$. For any $x \in X \cap T$, choose the cluster $(x, *, *)$ in $SC$; similarly for $y \in Y \cap T$ and $z \in Z \cap T$, choose the clusters $(*, y, *)$ or $(*, *, z)$ respectively in $SC$. Since $T$ is a vertex cover, $SC$ will cover all tuples in $S$ and has size $\leq M = k$.
\par
(if) Suppose $S$ has a non-trivial solution $SC$ of size $\leq k = M$. The clusters in $SC$ can have $*$ in zero, one, or two positions (all three positions cannot be $*$ since $SC$ is a non-trivial solution). We will argue that any cluster in $SC$ can be replaced by a cluster with two $*$ and a vertex from $G$ forming another feasible non-trivial solution without increasing the size of $SC$ (the size may decrease). Consider any tuple of the form $t = (x, y, Z_{xy})$ in $S$ (the other two cases $(x, Y_{xz}, z)$ and $(X_{yz}, y, z)$ follow similarly). If $t$ is covered by a cluster of the form $(x, y, Z_{xy})$, $(x, y, *)$, $(x, *, Z_{xy})$, $(*, y, Z_{xy})$, or, $(*, *, Z_{xy})$, such clusters cannot cover any other tuple in $S$ since $Z_{xy}$ is unique, so replace such clusters by $(x, *, *)$ or $(*, y, *)$. After this is repeated for all tuples in $S$, the only types of clusters remaining in $SC$ be of the form $(x, *, *)$, $(*, y, *)$, or $(*, *, z)$, which corresponds to a vertex cover in $G$, and the size of the solution has not increased.
\end{proof}
}
}







%%%%%%%%%%OLD INDEPENDENT SETS



\cut{
%\begin{minipage}[width=0.45\textwidth]
%      \includegraphics[width=0.45\textwidth]{general-graph}
%\end{minipage}



\begin{figure}
\subfigure[\small Graph formulation]{\label{fig:general-graph}\includegraphics[width=0.45\linewidth]{general-graph.pdf}}~
\subfigure[\small Reduction from independent set]{\label{fig:indepset}\includegraphics[width=0.45\linewidth]{indepset.pdf}}
%\caption{\small Graph formulation}

%    \hfill
%    \subfloat[{\small Reduction from independent set}\label{fig:indepset}]{%
%      \includegraphics[width=0.45\textwidth]{indepset}
%    }
%    \caption{Dummy figure}
%    \label{fig:dummy}
\end{figure}

\textbf{A simple graph formulation:} The optimization problem stated in Definition~\ref{def:formalDef} has multiple constraints, and therefore, it is not surprising that the problem is NP-hard. In fact, there is a simple graph formulation of this problem where we have two sets of vertices, $V_c$ for clusters and $V_t$ for elements, with edges in between if a cluster covers an element. In addition, there are edges between clusters if either one of them covers the other, or if their distance is $< D$. In this setting, our problem can be considered as finding a subset of the clusters with maximum value (i) of size at most $k$, (ii) forms an independent subset of $V_c$ (no edges between any two clusters), and (iii) covers top-$L$ elements\footnote{Our problem has a coverage constraint but is different from the max-cover problem (cover maximum elements using $k$ sets) in terms of the cost -- if two sets cover the same element, the element is counted once in the max-cover problem, but will contribute the overall score twice in our problem.}.    Even ignoring $k$ and $L$ (only one element in $V_t$ with weight 1 covered by all clusters in $V_c$, and $k = |V_c|, L = 1$), there is a simple reduction from the independent set problem that makes this formulation NP-hard. However, if we take the semilattice structure of the clusters into account, this reduction does not work.
\par
\red{THE COMPLEXITY OF THIS PROBLEM IS UNSOLVED -- look at the related work folder under Box -- finding a max weight antichain in a lattice is solvable in poly-time from the min-flow max-cut theorem -- see Mohring85, page 66-67. However, the complexity of this problem is unclear :~ find  a max weight antichain among the one having total width at most k -- see the np-hard.pdf in the related work folder -- but this is an old paper (1996) -- need to look for newer papers that have cited this paper}.\\

\yuhao{I am adding the NP-hardness proof here}.\\

\begin{theorem}
This.....non-trivial....
\end{theorem}

\begin{proof}
Proof here
\end{proof}


}









\cut{



\par


In this section, we present a simplified formulation of the optimization problem given in Definition \ref{def:formalDef} for investigating its complexity. The input of the problem is a graph $G(V_c, V_t, E_{cc}, E_{ct})$ where $V_c$ denotes clusters and $V_t$ denotes tuples of $S$. If one cluster covers another or their distance less than $D$, they are connected by an edge $e \in E_{cc}$. If one tuple is covered by a cluster, they have an edge $e \in E_{ct}$. The output of the problem is a subset $V_c^{'}$ of $V_c$ that contains $k^{'}$ vertices where $k^{'} \leq k$ such that:
\begin{itemize}
\item The vertices in $V_c^{'}$ should have edges with top-$L$ $v \in V_t$.
\item $\forall i,j \in [1, k^{'}]$, $i \neq j$, $(v_i, v_j) \notin E_{cc}$, i.e.\ $dis(v_i, v_j) \geq D$ and $v_i$ does not cover $v_j$ and vice versa.
\item $V_c^{'}$ have the largest $score$ among all the satisfied set in $V_c$.
\end{itemize}

\begin{example}
\input{problemGraph}
Figure \ref{instance of problem} shows an instance of our problem. In this instance, we only have two attributes. And for each attribute, it only has two different values.
\end{example}

\subsection{NP-hardness}
In this section, we show NP-hardness of the subset selection problem defined previously. Since finding clusters on a set of attributes is a special case of this subset selection problem, this does not imply NP-hardness of the optimization problem given in Definition 3.3. We are currently working on strengthening the NP-hardness result to this special case.
\input{proveGraph}
\par
We reduce our problem from the maximum independent set problem: given a graph $G^{'}(V, E)$, find a subset of vertices $V^{'} \subseteq V$ such that there is no edge between any two vertices in $V'$. We will construct an instance of our problem. Let $V=V_c$, $E=E_{cc}$. We add a new vertex $v \in V_t$ as only element in $V_t$ and it has edges with all the $v_c \in V_c$. The vertex $v$ has a value of 1. All the vertices that connected with $v$ has the same value which means $\forall v_c \in V_c$, the weight $w_{v_c}$ is 1. In our problem, set $k \leq \left|V_c\right|$ and $L=1$. Figure \ref{prove graph} shows the construction. We show that if the independent set problem has a solution of size $N$, then our problem has a score of $N$ and vice versa. (1) Suppose there is an independent set $V'$ of size $N$ in $G^{'}$. We select vertices in $V^{'}$ as the output clusters of our problem, which is a feasible solution with total value $N$. (2) Suppose we selected a subset $V_c^{'}$ as the solution of our problem. As every vertex in $V_c$ has the same value, and  suppose the size of $V_c^{'}$ is $N$, the total weight of $V_c$ is $N$. Since $V_c^{'}$ is a feasible solution, it must be an independent set, which gives a solution of the independent set problem of size $N$. The construction time is polynomial, so we prove that this problem is NP-hard.

Note that, if the $k$ is a constant, the problem can be solved in polynomial time. This is because we can check the total value of all subsets in $V_c$ whose size is at most $k$ in $O(n^k \times poly(n, k))$ where $n=\left|V_c\right|$. However, it is still hard to compute. For example,  we assume that $k=10$, the domain size of each attribute is 9, and the number of attributes is 4. Considering the ``don't care'' values $*$ for attributes, the number of clusters n can be $10^{4}$, and $n^k$ is $10^{40}$. In our experiments, we will compare our algorithms with the brute force method (given in Algorithm \ref{instance of problem}) experimentally.

%\begin{itemize}
%\item Let the $\val$ of $e \in V_{ct}$ equals to a constant number, for example, one.
%\item Let the value of vertex $v_c \in V_c$ equals to the largest value of $v_t$ that has edges with the $v_c$.
%\item Let $k=\infty$
%\item Let the $score$ of the $C^{'}$ as the sum of the value of $v_c \in C^{'}$.
%\item Based on the two items above, if we select $v_c$ as many as we can, the $score$ of the set is maximum.
%\item So our problem comes to a maximum indepedent set problem.
%\end{itemize}
%deduction from some form of independent set problem?
%set d=1, so the only constrain of $E_{cc}$ is domination.
%how to select any independent set that cover all the top-$L$? Let value to be same, say every value of tuple is 1. 
%Do I need to set $L$ = 1?? No, Every $V_c$ now have a weight
%The weight is max(value of tuples). The score of the set is the max(value of clusters).
%can we select independent set that size of k? to independent set?

%(How to deduct from set cover problem?)

}

==> discussion.tex <==
\red{
\section{Discussion}

\subsection{Discussion against decision trees}
Decision tree is a widely used machine learning approach for classification and finding features. However, decision tree is designed for n-ary objective functions, where $n$ is finite. While our problem is not an n-ary problem - we do not explicitly determine which values are wanted and which are not. Relatively high valued elements are not expelled even if they do not belong to top-$L$ elements. As a result, it would be hard to determine the cutoff values needed in decision tree. That is why we did not choose decision tree as our approach to investigate our problem.

\subsection{Automatically choosing parameters}
We have been considering about choosing default values for the users to make their journey even easier. However, we found it can be misleading - the system doesn't know the user's actual demand. For a same input sql query, different users are highly likely to have different expectations. For example, some may look for high-valued clusters regardless of other conditions, while others may be interested in diverse clusters with moderate values. Ultimately, the decisions should be made by the user. We would like to help them by providing the guidance visualizations- instead of doing for them - to their destinations.

}

==> expt-qualitative.tex <==
\subsection{Qualitative Evaluation with Other Related Approaches}\label{sec:expt-compare-others}
For the query in Example~\ref{eg:intro}, we here compare the results adapting approaches in three related papers \cite{JoglekarGP16, QinYC12, drosou2012disc} that are most relevant to this work (\ie, consider both summarization and diversification). Comparison with the MMR-based $\lambda$-parameterized diversification framework (no summarization) from  \cite{Vieira+ICDE2011} can be found in the full version \cite{fullversion} due to space limitation. Since our framework is not directly comparable with \cite{JoglekarGP16, drosou2012disc, QinYC12} for running time evaluation, we compare the results (for \maxval) qualitatively by using the brute-force or an efficient algorithms from these papers using $k = 4$, $D = 2$, and $L = 10$.
\subsubsection{Comparison with smart drill-down \cite{JoglekarGP16}}\label{expt:smart-drill-down} 
 The goal in \cite{JoglekarGP16} is to find an ordered set of $k$ rules (clusters with $*$ in our framework) $R$ with maximum score  ${\tt score(R)  = \sum_{r \in R} MCount(r, R) \times W(r)}$, where the marginal count ${\tt MCount(r, R)}$ denotes the number of tuples covered by $r$ but not covered by preceding rules in  $R$, and $W(r)$ denotes the number of non-$*$ attributes in $r$. The two parameters focus on diversity (by preferring rules with high ${\tt MCount}$) and good-ness (by preferring more specific rules) of rules. To compare it with our framework with {\em relevance} (summarizes aggregate results where tuples have values), we update the scoring function as ${\tt score(R)  = \sum_{r \in R} MCount(r, R) \times W(r) \times \val(r)}$, where $\val$ denotes the average value of the elements covered by $r$ that are uncovered so far by previous rules. Our framework also considered {\em coverage} of top-$L$ elements, so we evaluated a greedy algorithm (shown to perform well in \cite{JoglekarGP16}) on two inputs: (i) all elements in the aggregate query results, and (ii) top-$L$ elements and obtained the following results:
 
 \begin{center}
 {\centering
{\scriptsize
\begin{tabular}{|c|c|c|c||c|}
\hline
{\tt hdecade} & {\tt agegrp} & {\tt gender} & {\tt occupation} & {\tt \bf avg score}   \\\hline\hline
%& {\tt decade} & {\tt range} & & & \\\hline
\rowcolor{Gray}
\multicolumn{5}{|c|}{{\bf Smart drill-down on top-10 elements}}\\\hline
* 	& 20s 	&  M 	& * 	& 3.47 \\\hline
* 	& 10s 	& M  	& Student 	& 3.63 \\\hline
1995 	& 30s 	& F  	& Educator 	& 3.70 \\\hline\hline
\rowcolor{Gray}
\multicolumn{5}{|c|}{{\bf Smart drill-down on all elements}}\\\hline
1995 	& *  	&  M 	& * 	& 3.18 \\\hline
* 	& 20s 	& M  	& *  	& 3.47 \\\hline
1995 	& * 	& F  	& * 	& 3.24 \\\hline
* 	& 10s 	& M  	& Student 	& 3.63 \\\hline
\end{tabular}
}
}
\end{center}
Comparing the above tables with Figure~\ref{fig:eg-intro-clusters} and \ref{fig:eg-intro-two-layer}, we see that the average score of the rules or clusters is much less than our output. Although the above rules capture {\tt (20, M)} that is prevalent in the top-10 results in Figure~\ref{fig:eg-intro-top-bottom}, it is not a characteristics of the top-valued elements; \eg, elements ranked 44, 46, 49 (in total 18 out of 50 tuples) satisfy this rule leading to a low score.
% due to these ``false positives''. 

\subsubsection{Comparison with diversified top-$k$  \cite{QinYC12}}\label{expt:dtopk}
Given the elements with scores, using our terminology, the goal in \cite{QinYC12} is to find at most $k$ elements such that the distance between any two chosen elements is at least $D$ and the sum of scores is maximized. This notion considers {\em diversity} and {\em relevance}. To also include coverage like ours, we ran it on top-$L$ elements and got the following answers (by a brute-force implementation since the goal was qualitative evaluation). We show both actual value of the representative elements ({\tt score}) as well as the average value of elements within distance $D-1$ of these chosen elements ({\tt avg score}) below since intuitively the chosen elements cover these elements.

 \begin{center}
 {\centering
{\scriptsize
\begin{tabular}{|c|c|c|c|c||c|}
\hline
{\tt hdecade} & {\tt agegrp} & {\tt gender} & {\tt occu.} & {\tt score} & {\tt \bf avg score}   \\\hline\hline
\rowcolor{Gray}
\multicolumn{6}{|c|}{{\bf Diversified top-$k$ on top-10 elements}}\\\hline
1975 & 20s 	&  M 	& Student 	& 4.24 & 3.71 \\\hline
1980 	& 20s 	& M  	& Programmer 	& 4.13 & 3.77 \\\hline
1980	& 10s 	& M  	& Student	& 3.97 & 3.69 \\\hline
1995 	& 30s 	& F  	& Educator	& 3.70 & 3.52 \\\hline
\end{tabular}
}
}
\end{center}
Although \cite{drosou2012disc} optimizes for a different optimization goal, the above results illustrate that it does not perform well for our goal of summarization of top-valued elements with diversity. {\em First,} the average values of the ``clusters'' formed by the representative elements shown above are less than the values given by our approach in Figure~\ref{fig:eg-intro-clusters}. These chosen values include the original top-10 elements within distance 1, but also include many elements with low values within such circle. For instance, the first element above covers 6 elements (including itself) and covers the 28th element with value 3.12. {\em Second,} the representative of a cluster is one of the original elements, and we are not getting summarized common properties of the cluster using $*$-attribute values. %\red{what else}?

\cut{

1975	20	M	Student	4.23943661971831	avgVal:3.7097565996942751 (5 in total)
1980	20	M	Programmer	4.130434782608695	avgVal:3.7703056061603691 (6 in total)
1980	10	M	Student	3.9649122807017543	avgVal:3.6860677117440098 (5 in total)
1995	30	F	Educator	3.6984126984126986	avgVal:3.5225362725362725 (3 in total)

}
 
\subsubsection{Comparison with DisC diversity \cite{drosou2012disc}}\label{expt:disc}
Given the distance parameter $D$ and a set of elements $P$, the goal of  \cite{drosou2012disc} is to find a {\em DisC diverse subset} $S^*$ of minimum size such that each element in $P$ is at most distance $D$ from some element in $S^*$, and no two elements in $S^*$ are within distance $D$ of each other.  Like \cite{QinYC12}, this diversity notion naturally includes summarization, since an element can be assigned to the {\em cluster} corresponding to a point in $S^*$ at distance $\leq D$. To also include the notion of {\em relevance} and {\em coverage of top-$L$}, we ran it too on top-$L$ elements (a brute-force implementation) and obtained the following results. Like \cite{QinYC12},  \cite{drosou2012disc} gives clusters with smaller scores than ours (.\eg, the first tuple ``covers'' eight elements where the last one is of rank 28 and has value 3.31), and do not exhibit the common properties by $*$ values. 
These qualitative comparisons illustrate the effectiveness of our approach. % for summarizing top aggregate query results.

 \begin{center}
 {\centering
{\scriptsize
\begin{tabular}{|c|c|c|c|c||c|}
\hline
{\tt hdecade} & {\tt agegrp} & {\tt gender} & {\tt occu.} & score & {\tt \bf avg score}   \\\hline\hline
\rowcolor{Gray}
\multicolumn{6}{|c|}{{\bf DisC diversity on top-10 elements}}\\\hline
1980 & 20s 	&  M 	& Student 	& 3.91 & 3.81 \\\hline
1985 	& 10s 	& M  	& Student 	& 3.76 & 3.66 \\\hline
1995 	& 30s 	& F  	& Educator 	& 3.70 & 3.52 \\\hline
1985 	& 20s 	& M  	& Engineer	& 3.65 & 3.62 \\\hline
\end{tabular}
}
}
\end{center}
% \red{WHAT ELSE?}

\cut{
DisC distance = 1: 
1980	20	M	Student	3.907514450867052	avgVal:3.8096829243893948 (8 in total)
1985	10	M	Student	3.764705882352941	avgVal:3.6571964005179678 (5 in total)
1995	30	F	Educator	3.6984126984126986	avgVal:3.5225362725362725 (3 in total)
1985	20	M	Engineer	3.6451612903225805	avgVal:3.6199925013343510 (6 in total)
}




\cut{ table of neighbors
Disc D= 1 (1980 20 M Student)
1975;20;"M";"Student";4.2394366197183099
1980;20;"M";"Programmer";4.1304347826086957
1980;10;"M";"Student";3.9649122807017544
1980;20;"M";"Student";3.9075144508670520
1980;20;"M";"Engineer";3.8333333333333333
1985;20;"M";"Student";3.7631578947368421
1990;20;"M";"Student";3.3259668508287293
1995;20;"M";"Student";3.3127071823204420


DTOPK D=2 (1975 20 M Student)
1975;20;"M";"Student";4.2394366197183099
1980;20;"M";"Student";3.9075144508670520
1985;20;"M";"Student";3.7631578947368421
1990;20;"M";"Student";3.3259668508287293
1995;20;"M";"Student";3.3127071823204420
}






==> response.tex <==
\section*{Response Letter for Paper 700}\label{sec:response}
We thank the reviewers for their clear and constructive reviews.  We
have addressed all comments from the reviewers.   Updates made in response to specific
comments are color coded as follows:
% (some comments are common to more than reviewers.)
\begin{itemize}
\itemsep0em
\item \reva{Reviewer 1 in RED}
\item \revb{Reviewer 2 in BLUE}
\item \revc{Reviewer 3 in MAGENTA}
%s\item \revd{Metareview in CYAN}. 
\end{itemize}

%\par 
% We have highlighted some specific changes asked by the reviewers using the following
% colors in the paper. 

%\begin{itemize}
%\itemsep0em
%	\item {\color{red} Updates for comments from Reviewer 1:  {RED}}
%	\item {\color{blue} Updates for comments from Reviewer 2:  {BLUE}}
%	\item {\color{magenta} Updates for comments from Reviewer 3:  {MAGENTA}}
%	\item {\color{cyan} Updates for comments from Reviewer 4:  {CYAN}}
%\end{itemize}
%Other, general improvements throughout the paper are not highlighted.
%they affect Sections 2.3 and 3.1 (page 5), Sec 5.1 (pages 9-11), and
%Sec 6 (page 12, expanded into discussions).
We explain below how we addressed specific comments. We copy the comments for required changes for easy reference.

% The changes asked by the reviewers are written in \textbf{bold} below, and our responses with pointers to the changes
% are written as \ans{$\cdots$}.

\subsection*{Meta-Review}
%\begin{itemize}[leftmargin=*]
%\itemsep0em
 \ques{Thank you for your submission to PVLDB. While the reviewers appreciate
your research results, they had concerns which they felt could be
addressed in a revision. We encourage you to revise your paper taking
into consideration the reviewer comments, and submit an improved
version of the manuscript.

A key weakness is that the paper does not
really show that the proposed approach is useful -- you must provide
case studies to show this.}

\ansd{We have added a detailed user study section to evaluate the
  utility of user-specified parameters in our approach, and to compare
  our approach with our best effort of adapting an existing technique
  to our setting (based on decision trees). We also reported the
  feedback from the visitors of the demonstration of the system at
  SIGMOD 2018.}

\ques{In addition, you must also address the requirements listed in the individual reviews.}
 
 \ansd{We have addressed  the comments in the individual reviews as listed below.}


%\end{itemize}

\section*{Changes and explanations for \color{red}{Reviewer 1}}
%\subsection*{Major changes}
%\textbf{(1) ``Added a user study to evaluate the benefits of the assumed constraints as well as comparison with result of decision tree''}
\begin{itemize}[leftmargin=*]
\itemsep0em
%\item\textbf{(R1-W1)}  \ques{The query under study is contrived with a very limited set of applications. ...}
\item\textbf{(R1-W1)}  \ques{A user study is needed to evaluate the benefits of the assumed constraints and in turn the summarized data.  (details below).}~~~~
\ansa{We have added a detailed user study section to
evaluate the utility of user-specified parameters and 
to compare our approach with decision trees in our approach (Section~\ref{sec:user-study}). We also reported the feedback from the visitors of the demonstration of the system at SIGMOD 2018.}


\item\textbf{(R1-W2)}  \ques{The work makes some unrealistic assumptions about the underlying model, which limits its applicability (details below).}~~~~\ansa{Please see R1-D1 (2) below.}

\item\textbf{(R1-W3)}  \ques{The work is rather incremental as several schemes have been proposed for the relevance+diversity problem (details below).}~~~~\ansa{We have compared this work qualitatively with other approaches as discussed in the related work (and in the extended version). Please also see R1-D5 below.}

\item\textbf{(R1-D1)}
 \ques{In the end, the work is formulated as an optimization problem with constraints and objective to maximize. However: 1) it is not clear what is the relationship between those objectives+constraints on the user experience,}
 \ansa{We have now evaluated this in the user study (please see R1-D2 below).}
 
 \ques{ 2) the work proposes several straightforward greedy heuristics to solve that optimization problem, which rather limits the novelty.}~~~~
\ansa{
We have revised the introduction to explain our contributions better
and highlight the following:

(a) With three competing constraints, we have designed two heuristics
(bottom-up and fixed-order) with one demonstrating better efficiency,
and the other with better quality. Our final solution is a hybrid
algorithm incorporating these two heuristics.

(b) However, the straightforward implementations of these heuristics
did not give interactive speed of our algorithms, which we solved by
developing multiple optimizations (precomputation, batch computation,
interval tree data structure, incremental updates, using hash values
for non-numeric fields etc.) (also see
Section~\ref{sec:guidance}). Eventually we achieved 30x-1000x speed up
from these optimizations, which helped us achieve our goal of
interactive speed.

(c) As an additional feature, these optimizations provided the users a
visual guide for parameter selection showing a holistic view of how
the objective varies with different choices of parameters, and
identify ``flat regions'' (uninteresting for parameter changes)
vs. ``knee points'' (possibly interesting for parameter changes).

(d) We also provided the comparison view to visually see the change from a previous run, and provided solutions to an optimization problem to minimize clutters in the flow diagram. However, due to the new section on user study, these results had to be moved to the full version \cite{fullversion}.}
%Updated notation - moved definitions to a table, clarified notations throughout when used in paper.}

\item\textbf{(R1-D2)}
\ques{Regarding \#1 above, a user-based case study appears essential to validate the hypothesis that the output of that optimization problem is of some benefit to real users in a real application scenario. Otherwise, it is a pure optimization problem, in which the constraints and objective could be artificial and disconnected from real applications. }~~~~
\ansa{We have added a new user study section (Section~\ref{sec:user-study}). In the user study, we have evaluated (a) variations of choices for different parameters ($k, D$), (b) comparison with the output returned by a decision tree classifier for top-$L$ elements, and (c) usefulness of our visual guide for parameter selection (usefulness of comparison with the previous setting is discussed in the full version \cite{fullversion}. 
\par
As a summary, we observed the following: (1) Different users may prefer solutions with different values of $k$ and $D$, and there may not be a unified preference among users (the third parameter $L$ is completely user's choice about how many original top elements the clusters should cover). (2) The users prefer our solution compared to more complex output by decision tree, and can answer tasks more efficiently and accurately  with our solutions. (3) Even though in our experiment a higher $D$ provides better performance, still a decent amount of users prefer the more detailed result given by a lower $D$. (4) We informally asked the visitors of our demonstration at SIGMOD 2018 about the utility of our visualizations and the response was highly positive.

%\green{CHECK AND REVISE}
}
%\@YUHAO: PLEASE COMPLETE THE ABOVE FROM THE USER STUDY. DONE.}
%. We defined our use case better, and added a longer list of examples and queries in the experiments section, see Section 8.1 - Relative System Performance.}

\item\textbf{(R1-D3)}  
 \ques{Regarding \#2, the space of heuristics for solving this problem is potentially large. In turn, it would be helpful to: 1) provide some insights into the analytic performance bounds of the proposed heuristics, }
 \ansa{Due to multiple constraints ($k, L,D$, incomparability) and complex objective (average value of the covered tuples), we do not have a non-trivial approximation bound -- we have added it as a future direction  (Section~\ref{sec:conclusions})}
 
 \ques{and  2) compare to a large set of baselines, including basic ones such as: clustering and random.}
  \ansa{We have added the following new comparisons in Figures~\ref{fig:brute-force-time} and~\ref{fig:brute-force-val} in Section \ref{sec:perf-params}.  Basic clustering algorithms and random clusters do not meet our solution constraints.  Therefore, for fair comparison, we incorporated them as variants of our \fixedorder\ (essentially letting \fixedorder\ to fix any constraint violations).  In the random variant, we choose $k$ out of top-$L$ elements at random as initial clusters; in the `$k$-means' variant, we first run the $k$-means clustering algorithm on the top $L$ tuples, find the tightest pattern covering all members in each cluster, and use these as the initial clusters.  \fixedorder\ then proceeds these initial clusters followed by the top $L$ tuples.  As shown by the results of the experiments, these variants do not improve solution quality, introduce uncertainty, and slow down the processing time.}

\item\textbf{(R1-D4)}  
 \ques{The paper assumes an oversimplified binary model for measuring the distance/dissimilarity between tuples. However, that model would be insufficient for dimensions with numerical values, in which some variant of Lp norm would be more suitable. }~~~~
\ansa{We agree with the reviewer that for numerical values a more fine grained distance function like using $L_p$ norm would be more meaningful. However, we mainly focused on categorical values in this paper. We have now clarified it in Section~\ref{sec:prelim} and added other distance function as possible directions for future work (Section~\ref{sec:conclusions}), which is likely to require a new set of techniques.}

\item\textbf{(R1-D5)}  \ques{ It is not clear to me what is the impact of aggregation and why it is considered a new contribution of this paper? In particular, once the aggregate query is answered, the resulting tuples are basically points in a data space. Hence, existing work on non-aggregated values becomes directly applicable. Along the same lines, the paper assumes that the aggregate value is an indication of the importance. But is that always the case? }~~~~
\ansa{%CHECK AND EDIT!!!
The aggregate queries are used to have a score for the output tuples (to measure relevance or importance as in a top-K query), and our goal is to summarize the high valued tuples according to this score subject to additional constraints. In previous work in the literature (e.g. in \cite{Vieira+ICDE2011}, which does not focus on summarization) a measure for relevance has been used. As we have discussed in the related work section and in the qualitative evaluation in our extended version \cite{fullversion}, the previous papers had different objectives and did not consider all of relevance, diversity, coverage, and summarization simultaneously, and those papers or their adaptations do not meet our goal. However, the relevance measure or score does not have to come from an aggregate query, and can be given, for instance, by a domain expert. We have clarified this in Section~\ref{sec:prelim}.}

%\green{CHECK AND REVISE}}



%\cut{ 
%We analyze some clustering algorithms and do the comparison in the related work section in order to show why those existing works are not perfectly directly applicable. What we proposed is the way that we think the best applicable in the scenario we described in the introduction section. THE IMPORTANCE STUFF I'M NOT SURE HOW TO RESPOND TO THAT...\\
%
%DISCUSS!! EACH TUPLE IS ASSOCIATED WITH A VALUE/SCORE COMING FROM AGGREGATE QUERY -- CITE DIVESH SRIVASTAVA PAPER THAT CONSIDERS SOME OBJECTIVE -- although we considered aggregate, we can handle any table with some measure attribute -- add in the conclusions.\\
%
%TODO FOR SUDEEPA FOR FIRST PASS}
%}\yuhao{Checked and looks fine for me.}


\item\textbf{(R1-D6)}  \ques{I find the motivating/running example very confusing, especially when it comes to the statement: “but it is misleading, since a closer look at Figure 1a reveals that many tuples with low values (49th, 46th, 44th) share this property too, suggesting that male viewers in their 20s may or may not give high rating to the adventure genre.”. so how to avoid that? especially that the formulated optimization problem will not recognize that case given constraints L and the goal of maximizing average relevance/score.}~~~~
\ansa{The objective function to maximize ``average'' score of tuples contained in all the clusters will try to avoid this case, since the cluster for (20, M) will have many low-valued tuples and therefore will reduce the value of the objective function. Indeed, it can be seen from Figure~\ref{fig:eg-intro-clusters} that (20, M) has not been chosen in the solution and more specific clusters for the high-valued tuples have been chosen. We have further clarified it in the introduction (page 2).}

\item\textbf{(R1-specific revisions)}
  \ques{D1 to D6}
\ansa{As described above, all are addressed.}
\end{itemize}

\section*{Changes and explanations for \color{blue}{Reviewer 2}}
%\subsection*{Major changes}


\begin{itemize}[leftmargin=*]
\itemsep0em
\item\textbf{(R2-W1)}  \ques{There are a few restrictions on supported queries (apparent in the example and the experimental evaluation) that need explanation. Ideally, the set of queries supported should cover a wide range of typical data scientist aggregate queries.}~~~~
  \ansb{(1) We actually have no restrictions on the supported SQL queries as long as the output is associated with a score or value signifying the relevance or importance of output tuples. This is because we take the output table of the SQL query as input, and then apply our clustering algorithm with constraints that aims to maximize the average score of the covered tuples. Therefore, although we have used {\tt average} in the example queries, we are oblivious to more complex aggregate queries or other aggregate functions.
    
  (2) Further, although we have used average score of covered tuples as our objective (since this is simple as well as captures properties common to high-valued tuples, whereas using `sum' can include many low-valued tuples in the clusters), our algorithms can support other more complex aggregate functions in the objective (although the NP-hardness proofs from this work in our full version\cite{fullversion} may not hold for other objectives).
  
We have explained these further in Section~\ref{sec:prelim} and in conclusions (Section~\ref{sec:conclusions}).

\cut{Theoretically it makes no difference to the proposed algorithms for the three common aggregate SQL function - COUNT(), AVG() and SUM(), since our algorithms consider the aggregate result table as the input and do calculations upon that table. NOT SURE IF THAT EXPLANATION IS ENOUGH, OR WE SHOULD ADD CONTENT IN MAIN CONTEXTS. -- we are oblivious to more complex aggregate function in the aggregate query -- we can also replace the average objective by more complex objective/different way of combining the solution quality (although the NP-hardness proof will not work.)}
}
\item\textbf{(R2-W1)}  \ques{Some definitions / descriptions / notations could be more precise or consistent (see D1, D2, D4).}
\ansb{Addressed below in R2-D1, R2-D2, R2-D4.}
%\end{itemize}
%\subsection*{Other changes and explanations}
%\begin{itemize}[leftmargin=*]
%\itemsep0em
\item\textbf{(R2-W3)}  \ques{The presentation of the experiments (graphs) and also screenshots could be improved to increase readability. As is, they are too small / too cluttered.}~~~~
\ansb{We have removed the screenshots because of space constraints due to additional content, and since they appear in our SIGMOD 2018 demo paper \cite{qagviewdemo2018} -- this is now mentioned in Section~\ref{sec:experiments}. We have made the graphs bigger and fonts clearer.}

\item\textbf{(R2-D1)}  \ques{Definition 3.1: $t[A_i] \neq t[A_i] \rightarrow $ I suppose one should be $t'$.}
\ansb{Correct. It is $t'$ and fixed.}

\ques{ Also, the definition leaves room for interpretation: "one of the values is *" vs at least one of the values is *".}
\ansb{We have changed it to ``at least one of the values is *''.}
%\ansb{(1) It is $t'$ and fixed. (2) It should be "at least one of the values is *" as explained in the equation follows in 3.1.}. \ansa{ABOUT (2): NOT SURE IF WE SHOULD MAKE THAT CHANGE... TODO FOR SUDEEPA}

\item\textbf{(R2-D2)}  \ques{Definition 4.1 - Incomparability: "No two clusters in O cover each other" $\rightarrow$ Do you actually mean one another? If it is each other, they would be equivalent in the sense that one cluster $C_1$ covers the tuples of cluster $C_2$ and vice versa. }~~~~
\ansb{Correct. We have rephrased it in Definition~\ref{def:problem} as ``No clusters in O cover any other cluster in O...''}
%Changed the way to present the sentence in 4.1 to avoid confusion. TODO FOR SUDEEPA}

\item\textbf{(R2-D3)}  \ques{The graphs in the experimental section should be improved to have the x-axis label at a position that is not mixed with the tick labels.}~~~~
\ansb{We have revised all our plots to make them clearer.}
%WORKING ON IT. ------TODO FOR YUHAO} \yuhao{Done.}


\item\textbf{(R2-D4)}  \ques{Use upper case and lower case letters consistently both in the text and the graphs (e.g., k vs K in Fig. 11, other occurrences as well).}~~~~
\ansb{%WORKING ON IT. TODO FOR YUHAO -- PLEASE USE small k, big L, big D\\
All are changed to $k, L, D$.}
%\yuhao{Done.}

\item\textbf{(R2-specific revisions)}
\ques{Please address all issues raised in the review, with special care on the three major weak points mentioned above. That is, (i) make definitions more precise and notation more consistent;}
\ansb{We have updated these as mentioned above.}

\ques{(ii) make improvements on the experiment and screenshot presentation to make them less cluttered and more readable.}
\ansb{We have updated the figures and removed the screenshot (appears in our SIGMOD 2018 demo paper \cite{qagviewdemo2018}) as described above.}
%\ansb{TODO FOR SUDEEPA}
\end{itemize}

\section*{Changes and explanations for \color{magenta} {Reviewer 3}}
%\subsection*{Major Changes}
%\begin{itemize}[leftmargin=*]
%\itemsep0em
%
%\end{itemize}
%
%\subsection*{Other Changes and explanations}
\begin{itemize}[leftmargin=*]
\itemsep0em
\item\textbf{(R3-W1 and R3-C1)}  \ques{Too many details are moved to the extended version of the paper.

The main shortcoming of the paper is that it tries to cover too many things within a limited page limit. This requires the reader to constantly refer to the extended version for many details (literally every section seems to refer to the full version at least once). Given that the visualization aspects as presented in the paper are weak (see comments below), one way of improving the exposition would be to remove the visualizing the differences in clusters part of the paper. This will provide enough space to include most of the other omitted details as part of the main paper. This will also focus the paper on the summarization problem itself, detailing how it will help interactive visualizations.}~~~~

\ansc{Due to space constraints and because of the new user study section, we did have to remove the section on visualizing two sets of clusters from the paper and defer it to the full version\cite{fullversion} (also, this visualization is discussed in our recent SIGMOD 2018 paper\cite{qagviewdemo2018}). We have updated the introduction accordingly.} % \green{REVISIT.}}
%\ansc{TODO FOR ALL  --- AFTER WE ADD ALL THE CONTENT -- PLANNING TO SAY THAT THE INTERACTICE EXPLORATION IS AN IMPORTANT ASPECT OF THIS WORK, SO WE WOULD LIKE TO KEEP IT IN THE PAPER.}

\item\textbf{(R3-W2)}  \ques{Qualitative aspects of the visualization (especially the comparison visualization) not discussed.}~~~~
\ansc{
In addition to the user study to evaluate our system and different parameters, we have conducted an informal user study during the demonstration of our system at SIGMOD 2018. We asked the visitors how they liked (1) the guidance visualization for helping them choose parameters, and (2) the comparison visualization for comparing with the previous run. The visitors liked the visualizations and we have reported our findings in Section~\ref{sec:us-sigmod} (comparison visualization related report is moved to our full version\cite{fullversion}).}

\item\textbf{(R3-C2)}  \ques{The figures showing the visualizations (Fig. 2,6,8) are difficult to read.}~~~~
\ansc{Old Figure~2 and 6 are now replaced by the new Figure~\ref{fig:intro-guid}, which has been made clearer.  Old Figure 8 showing the screenshot has been removed due to space constraint, which can be found in our SIGMOD 2018 demo paper \cite{qagviewdemo2018}.} %TODO FOR YUHAO}\yuhao{Done.}

\item\textbf{(R3-C3)}  \ques{Fig. 2: why isn't the line for $d = 2$ visible? (there are some lines missing in the other figures as well, e.g., only $d = 1,2$ are visible in Fig. 6 etc.).|}~~~~
\ansc{
%YUHAO: PLEASE SEE IF YOU CAN ADD ANOTHER GRAPH FROM THE DEMO WHERE BOTH LINES ARE VISIBLE.\\
We have replaced the old Figure 2 and 6 with the new Figure~\ref{fig:intro-guid}. %replaced it with a new figure - currently 
Some of the lines overlap -- e.g., in the new graph, lines for $D = 4, 5, 6$ overlap. We have added legends to make it clearer. Further, in our system, the user can click on the respective boxes to make a subset of the lines visible.}
% \green{REVISIT AFTER ADDING LEGENDS.}}
%The $D=2$ line is overlapped with the line for $D=1$ and it is now explained in the caption of Figure~\ref{fig:intro-guid}. If the user click on the legend of $D=1$ (which can hide the corresponding line), the $D=2$ line will be visible. This happens when clusters in the result set of $D=1$ already meets the condition of $D\geq2$. }
%\yuhao{Done.}

\ques{Also, to be consistent, it should be $D=1, D=2$ etc.}
\ansc{Done.}
%TODO FOR YUHAO -- PLEASE USE D1, D2 -- not d1, d2... . PLEASE MAKE THIS GRAPH MORE READABLE} \yuhao{Done.}

\item\textbf{(R3-C4)}  \ques{Section 2: "Other works...": At least some justification on why these works are not applicable in the given context should be mentioned.}~~~~
\ansc{Added in Section~\ref{sec:related}.}

\item\textbf{(R3-C5)}  \ques{4.1, shouldn't the denominator of avg(C) be $|Cov(C)|$?}
\ansc{That is correct. It is fixed.}

\item\textbf{(R3-C6)}  \ques{7.2: Why should $P_a$ be fixed? $O_a$ simply gives the clusters that were previously present, but why should its ordering be the same when visualizing the changes?}~~~~
\ansc{$P_a$ shows the clusters for the previous result and shares the same ordering as they presented in the cluster table. The intuition is that it might be easier for users to understand the connection if we keep the ordering for the previous results ($P_a$) static, rather than re-ordering both cluster sets. However, this section has been moved to our full version\cite{fullversion} as mentioned before.}

\item\textbf{(R3-C7)}  \ques{Fixed-order consistently performs better than others w.r.t average value for higher values of D. Why is this the case, when the whole argument about using Bottom-up / hybrid is to get better valued results?}~~~~
\ansc{
%TODO FOR YUHAO -- MAY NEED DISCUSSION. 
  In terms of average value, Fixed-Order and Bottom-Up may perform better in different parameter setting. For example, Fixed-Order performs better in Figure~\ref{fig:VaryK-val}, and Bottom-Up gets mostly higher values in Figures~\ref{fig:VaryL-val} and \ref{fig:brute-force-val}. However, one main advantage of Bottom-up is that it is amenable to batch computation for all values of $k$ and $D$ for a given choice of $L$, and therefore it helps in precomputation and in the generation of guidance view.
  
Since Fixed-Order is more efficient than bottom-up, therefore, the intuition behind the Hybrid algorithm is that its efficiency is similar to Fixed-Order making our approach interactive, while it can generate values for all $k, D$ and help in precomputation as well as the generation of the guidance view.

We have now explained this better in Section~\ref{sec:algorithms}.}
%\green{CHECK. YUHAO: SHOULD 'NOT' BE NOW? I DON'T UNDERSTAND THE LAST SENTENCE QUITE MUCH.}

\item\textbf{(R3-C8)}  \ques{Fig 12(a): there is an additional legend.}
\ansc{
Old Figure~12(a) is new Figure~\ref{fig:brute-force-val}. It was not an additional legend -  the lines for Bottom-Up and Fixed-Order were overlapping with each other. 
We have updated the legends to make it clearer.} 

\item\textbf{(R3-C9)}  \ques{8.5: While the quantitative numbers w.r.t. number of crossings etc. are fine, there are no figures showing how these visualizations actually look. The only examples shown are very simply ones with small values of k. Even with all these optimizations will the visualizations be too cluttered to be useful?} ~~~~
  \ansc{Due to space constraints, we had to move the section on visualization for comparing two executions to the full version (old Section 7 is removed and new section on user study - new Section~\ref{sec:user-study} is added).
    
However, to answer this question, Figures 9 and 10 in the previous submission  (these figures are now removed) are examples showing that what does it look like for different number of crossings. In terms of larger $k$, the plots may be more cluttered even with optimizations. However, $k$ = the number of clusters the user wants to examine is likely to be small and the optimizations are likely to work well. We have conducted an informal survey in our demonstration at SIGMOD 2018. The visitors considered the visualization for comparison useful, and 7 out of 18 visitors thought it was ``very useful'' while all the other 11 thought ``useful''.}
% for them. TODO FOR YUHAO --- NEED TO ADD OBSERVATION FROM THE USER STUDY AT SIGMOD HERE.}\yuhao{DONE.}

\item\textbf{(R3-C10)}  \ques{Minor comments. 
Abstract: "optimization" problem.}~~~~\ansc{Fixed.}

\ques{Page 3, Col 1: This features $\rightarrow$ feature}~~~~\ansc{Fixed.}

\ques{Page 5, Col 2: This distance $\rightarrow$ The}~~~~\ansc{Fixed.}

\ques{Page 6, Col 2: greedily merges a pair is given in... $\rightarrow$ "merges a pair, and is given ..."}~~~~\ansc{Rephrased and fixed.}

\ques{5.3: instead of $ck$, use $c \times k$ to avoid confusion that $ck$ is a new variable}~~~~\ansc{Done as advised.}
%\ansa{COMMENT:Temprorily untouched due to possible room restriction}

\ques{Page 9, Col 2: When solution is accurate, it is redundant to mention that it has approximation ratio = 1.}~~~~\ansc{This line is removed.}

%~~~~\ansd{}\ansa{COMMENT: we got this confusion from previous reviewers saying we don't have the ratio....}

\ques{Page 9, Col 2: Section ?? - typo}~~~~\ansc{Fixed (this sentence is now deleted).} 
%\ansa{COMMENT: that was random order part, and since it's not discussed anymore, I just deleted that sentence. TODO FOR SUDEEPA}

\ques{8.1: Figure 12a compares "the running times of" our algorithms with...}~~~~\ansc{Fixed.}

\ques{8.4: one seconds $\rightarrow$ "few seconds" or "one second"}~~~~\ansc{Fixed.}

\item\textbf{(R3-specific revisions)}
\ques{Fix C1 - C10}
\ansc{All are addressed as described above.}
\end{itemize}

%\section*{TEMPORARY COMMENTS FOR YUHAO}
%
%\red{
%\begin{itemize}
%\item Please change $d = 1, d= 2$ in the legends to $D$ in Figure 2. \yuhao{FIXED}
%\item Please use a different setting where both graphs are visible.
%\item Please change $K$ to $k$ in Figure 3. \yuhao{FIXED}
%\end{itemize}
%}




==> test.tex <==
\section{AAA}
\begin{lrbox}{\sqlexp}\begin{minipage}{\textwidth}
\lstset{language=SQL, basicstyle=\ttfamily, deletekeywords={year,month,action},tabsize=2}
\begin{lstlisting}[mathescape]
SELECT $\langle$ grouping attributes$\rangle$, avg(rating) as $\val$ 
FROM RatingTable 
GROUP BY $\langle$ grouping attributes$\rangle$
HAVING count(*) > 50 
ORDER BY $\val$ DESC
\end{lstlisting}
\end{minipage}\end{lrbox}
\resizebox{0.85\textwidth}{!}{\usebox\sqlexp}

==> visualization.tex <==
%****NOTICE***
%THIS SECTION IS NO LONGER IN VLDB2018. TEXT IN APPENDIX WILL BE A BETTER REFERENCE IF WE WANT TO RESTORE THIS SECTION OR AS A SUBSECTION.



\subsection{Visualizing Successive Solutions}\label{sec:visualization}
Figure~\ref{fig_sim} %and Figure~\ref{fig:newgui} 
shows how a user can inspect the clusters and the elements they contain in the form of tables in our framework.
However, for interactive exploration, it is also important that the user can see how the old solution changes to a new solution (if $k,  D, $ or $L$ is updated), since in some cases the change can be incremental, whereas in other cases, changing a parameter may give a complete new solution. To support this comparison, %we display the successive solutions and their overlaps (Section~\ref{sec:comparison_gui}), and formulate it as an optimization problem for a clean display (Section~\ref{sec:comparison_opt}).
\ansc{
we display the successive solutions and their overlaps in Figure~\ref{fig:viz-clean}.Each box corresponds to a cluster in the solution. The left hand side boxes (in green) are result clusters for the previous run, and the right hand side boxes (in yellow) are clusters under the current parameters. The width of each box is proportional to  the number of tuples contained in the cluster.
\cut{ %%inappendix
\footnote{This visualization shows some similarity with SANKEY diagrams that are widely used in the field of energy and material flow management\cite{schmidt2008sankey}. 
% In some sense our visualization can be considered as an variation of SANKEY diagram since both 
and provide flow from one set of objects to another. However, popular SANKEY diagram libraries (\eg, d3-sankey) focus more on managing placement among columns (horizontal positioning). For vertical positioning, they do multiple iterations to re-position objects to achieve a satisfying visualization. We do not need to consider multiple columns, and our visualization focuses on vertical positioning and ordering of objects}.
}
  Clusters connected with bands or ribbons contain shared tuples. We formulate it as an bipartite matching problem with a polynomial optimal solution\cite{geomans2009} to generate a clean visualization. A cluttered one is displayed in Figure~\ref{fig:viz-chaos}. Details can be found in \cite{fullversion, qagviewdemo2018}.}

\cut{ The thicker a band is in the middle, the more common tuples it contains The parts of the boxes in darker color correspond to the fraction of top-$L$ tuples contained in these clusters. Hovering the mouse over different regions shows details. 

We formulate it as an bipartite matching problem with a polynomial optimal solution\cite{geomans2009} to generate a clean visualization. A cluttered one is displayed in Figure~\ref{fig:viz-chaos}.
% for comparison with a clean visualization in Figue~\ref{fig:intro-vizcompare}. 
Details about problem formulation deferred to the extended version of this paper\cite{fullversion}.
}

%  Once the user issues a new set of attributes or a new input query, the result cluster table will change to the new solution set aligned by the average value of each cluster. It is a clean way to show the result to the user, but the down side is: the result clusters can change completely even if there is only a trivial change in the combination of attributes, for example, $L$ increase by 1. It is highly possible for the user to lose track of the connection between two adjacent results. In order to maintain the connection between two consecutive results, we provide the visualization for the result comparison.

\cut{
\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figures/vizCompareClean.png}
\vspace{-0.2cm}
\caption{\ansc{Solution comparison: clean visualization}}
\vspace{-0.3cm}
\label{fig:viz-clean}
\end{figure} 


\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figures/vizCompareChaos.png}
\vspace{-0.2cm}
\caption{\ansc{Solution comparison: cluttered visualization}}
\vspace{-0.3cm}
\label{fig:viz-chaos}
\end{figure}
}

\cut{

\begin{figure}[t]
\centering
\begin{minipage}[t]{.47\textwidth}
  \centering
 %\vspace*{\fill}
\subfloat[{\scriptsize Clean visualization}]{
\includegraphics[width=0.42\linewidth]{figures/vizCompareClean.png}~~~~
\label{fig:viz-clean}}
\hspace{0.02\linewidth}
\subfloat[{\scriptsize Cluttered visualization}]{
\includegraphics[width=0.42\linewidth]{figures/vizCompareChaos.png}~~~~
\label{fig:viz-chaos}}
\vspace{0cm}
\end{minipage}\hfill
\caption{Clean and cluttered visualizations.}
\label{fig:vis-comparison}
\vspace{-0.2cm}
\end{figure} 

}
% FIRST SUBSECTION IS MERGED INTO MAIN PART AND SECOND SUBSECTION IS MOVED TO APPENDIX (AND CUT HERE, BUT BASICCALY COPY PASTE). TAKE CARE OF IT IN FULL VERSION.


\cut{

\subsection{Visualizing Changes}\label{sec:comparison_gui}
An example visualization is shown in Figure~\ref{fig:viz-clean}. Each box corresponds to a cluster in the solution. The left hand side boxes (in green) are result clusters for the previous run, and the right hand side boxes (in yellow) are clusters under the current parameters. The width of each box is proportional to  the number of tuples contained in the cluster. Clusters connected with bands or ribbons contain shared tuples. The thicker a band is in the middle, the more common tuples it contains \footnote{This visualization shows some similarity with SANKEY diagrams that are widely used in the field of energy and material flow management\cite{schmidt2008sankey}. 
% In some sense our visualization can be considered as an variation of SANKEY diagram since both 
and provide flow from one set of objects to another. However, popular SANKEY diagram libraries (\eg, d3-sankey) focus more on managing placement among columns (horizontal positioning). For vertical positioning, they do multiple iterations to re-position objects to achieve a satisfying visualization. We do not need to consider multiple columns, and our visualization focuses on vertical positioning and ordering of objects}. The parts of the boxes in darker color correspond to the fraction of top-$L$ tuples contained in these clusters. Hovering the mouse over different regions shows details.

}

\cut{
An alternative representation is to have the height of the clusters proportional to the number of tuples they contain while having the same width. However, the current formulation gives an optimal algorithm for an \emph{optimal placement} minimizing problem (see Section~\ref{viz:problem}) when the alternative formulation leads to an NP-hard problem.
Section~\ref{viz:problem} gives an extended discussion on the ordering problem.
}


\cut{

\subsection{Optimizing Cluster Placement}\label{sec:comparison_opt}

A careful ordering of the cluster boxes helps in displaying a cleaner visualization comparing two consecutive executions. For instance, Figure~\ref{fig:viz-chaos} is an example where placement of the clusters (boxes) leads to more \emph{crossing} of the bands, whereas  Figure~\ref{fig:viz-clean} shows a better placement. The placement can have more effect when the number of clusters (the value of $k$) is larger. Therefore, we formulate the cluster placement problem as an optimization problem that intends to minimize crossing of the bands as follows.
%As a result, it is meaningful to align the clusters carefully for formulating as a placement problem in the next subsection. 

%\subsubsection{Definition}
\textbf{Optimization problem.~~} Let $\soln_a$ and $\soln_b$ denote the old and new set of clusters respectively in two consecutive runs containing clusters $\soln_a = \big\{ c_{a1},c_{a2},...,c_{am} \big\}$ and $\soln_b = \big\{ c_{b1},c_{b2},...,c_{bn} \big\}$. Let $m_{ij}$ denote the number of shared tuples between clusters $c_{ai}$ and $c_{bj}$, and $M$ denote the set of all such $m_{ij}$ values.
\cut{
The number of tuples in each cluster in $S_a$ is $L_a=\big\{ l_{a1},l_{a2},...,l_{am}\big\}$ and $L_b=\big\{ l_{b1},l_{b2},...,l_{bn} \big\}$.
The mapping between two cluster sets is built in the form of $m\times n$ matrix $M$, where $m_{ij}$ shows the number of shared tuples between cluster $c_{ai}$ and cluster $c_{bj}$. 
}
\cut{
The visualization has two columns of boxes representing two cluster sets - previous set on the left and new set on the right -  with bands from left to right connecting both sides. All clusters (boxes) share the same unit height $1$.
} 
We assume that the first clusters in both sides are placed at the same vertical position, and there are no gaps or overlaps  between two adjacent clusters on either side. Consider two orderings of clusters on the left hand side and right hand side respectively  in terms of their starting positions $P_a = {p_{a1},p_{a2},..,p_{am}}$ (a permutation of $[0, m-1]$), and $P_b = {p_{b1},p_{b2},...,p_{bn}} $ (a permutation of $[0, n-1]$). We define a weighted \emph{earth mover's distance}\cite{rubner2000earth} $d_{ij}$ between one left cluster $c_{ai}$ and one right cluster $c_{bj}$ to evaluate the amount of crossing due to a single band (from $c_{ai}$ to $c_{bj}$) as:
\[ d_{ij} = m_{ij}\times|p_{ai}-p_{bj}|\]
Since $\soln_a$ is the previous cluster set, $P_a$ is fixed and given. The goal of the optimization problem for this visualization is to output a good ordering $P_b$ for $\soln_b$, and is formulated as follows:
%The value of $p_{ai}$ denotes the starting vertical position of $c_{ai}$ in $S_a$ and $p_{bj}$ denotes the position of $c_{bj}$ in $\soln_b$. 

\cut{
For the ordering, we have
\[ \forall  o_{ai}\in O_a, o_{bj} \in O_b, o_{ai}\in N^0, o_{bi}\in N^0\]
\[ \forall o_{ai}\in O_a, \forall o_{bj} \in O_b, 0\leq o_{ai}<m, 0\leq o_{bj}<n\]
\[ \forall i'\neq i, o_{ai}\neq o_{ai'}\]
\[ \forall j'\neq j, o_{bj}\neq o_{bj'}\]
}


\begin{definition}\label{def:opt-place}
\textbf{Optimization for placement of clusters.~~} Given old and new clusters $\soln_a$, $\soln_b$, %$L_a$, $L_b$, 
their overlaps $M$, and ordering $P_a$ of the clusters on the left hand side, find an ordering $P_b$ of the clusters on the right hand side that minimizes
$D=\sum_{i=1}^{m}\sum_{j=1}^{n}d_{ij}$.
\end{definition}

\textbf{Optimal solution using bipartite matching.~}
The above optimization problem can be reduced to the minimum cost perfect matching problem in a complete bipartite graph as follows. We form a weighted complete bipartite graph $G(U \cup V, E)$, where the $n$ nodes in $U$ correspond to the $n$ clusters in $\soln_b$, and the $n$ nodes in $V$ correspond to the positions $1 \cdots n$. An edge $(u, v)$ denotes the possibility when cluster $c_{bu}$ is placed in position $v \in [1, n]$. The weight of the edge $(u, v)$ is the cost $\sum_{i=1}^md_{iu}$ = $\sum_{i=1}^m (m_{iu} \times |p_{ai} - (v-1)|)$ (if $c_{bu}$ is placed in position $v$, there will be $v-1$ clusters before it, and its position will be $v-1$), \ie, the total contribution of cluster $c_{bu}$ in the optimization objective in Definition~\ref{def:opt-place} if it is placed in position $v \in [1, n]$. Since $\soln_a$ and $P_a$ are given and fixed, this weight can be computed in polynomial time as a precomputation step for each cluster in $\soln_b$ and each position. A matching gives a positioning $P_b$ on the clusters in $\soln_b$, and the minimum cost perfect matching, which has a polynomial time algorithm\cite{geomans2009}, gives an optimal solution to our optimization problem. %The solution is accurate and the approximation ratio is 1.
\par
We also studied an alternative formulation of the above optimization problem, where instead of the \emph{width} of the boxes being proportional to the number of tuples in clusters, the \emph{height} is proportional to the number of tuples, \ie, the starting positions $P_a$ and $P_b$ are no longer permutations of $[0, m-1], [0, n-1]$ but also depend on the height of the individual clusters. However, we found that this variant is NP-hard by a reduction from the \emph{earliness-tardiness job scheduling problem}\cite{garey1988one}. The proof and details of this alternative formulation are deferred to the extended version of this paper.

}

\cut{ 
For the simplified problem, every single cluster in both sides takes up the same amount of space. The cost for a cluster $c_{bj}$ can be directly written as
\[ d_{j}=\sum_{i=1}^{m} d_{ij} =\sum_{i=1}^{m} \big( |h_{ai}-h_{bj}|\times m_{ij} \big)\] 
Since there is no gap between clusters and $S_b$ has to start at position 0, the simplified problem can be considered as there are a series of fixed size slots and all clusters should be placed into slots in order to get the minimized total distance. Thus we can convert this problem into a complete bipartite graph, with nodes left to be the clusters in $S_b$ and the right nodes to be the vacant slots that to be assigned. The value of edges between a left node ($c_{bi}$) and a right node (the $j^{th} slot$) is $v_{ij}$. The problem is now equivalent to the minimum weight perfect bipartite matching problem\citep{geomans2009}:
\[ Min\quad \sum_{i,j}v_{ij}x_{ij}\]
\[s.t. \sum_{j}x_{ij}=1\qquad i\in {1,2,...,n} \]
\[\sum_{i}x_{ij}=1 \qquad j\in {1,2,...,n}\]
\[ x_{ij}\geq 0 \]
According to M. Goemans's material\citep{geomans2009}, this problem has been proved to be strongly polynomial and has an algorithm which has the complexity upper bound to be $O(n^3)$.
}



